Language Models as Compilers: Simulating Pseudocode Execution Improves Algorithmic Reasoning in Language Models

Algorithmic reasoning refers to the ability to understand the complex patterns behind the problem and decompose them into a sequence of reasoning steps towards the solution. Such nature of algorithmic reasoning makes it a challenge for large language models (LLMs), even though they have demonstrated promising performance in other reasoning tasks. Within this context, some recent studies use programming languages (e.g., Python) to express the necessary logic for solving a given instance/question (e.g., Program-of-Thought) as inspired by their strict and precise syntaxes. However, it is non-trivial to write an executable code that expresses the correct logic on the fly within a single inference call. Also, the code generated specifically for an instance cannot be reused for others, even if they are from the same task and might require identical logic to solve. This paper presents Think-and-Execute, a novel framework that decomposes the reasoning process of language models into two steps. (1) In Think, we discover a task-level logic that is shared across all instances for solving a given task and then express the logic with pseudocode; (2) In Execute, we further tailor the generated pseudocode to each instance and simulate the execution of the code. With extensive experiments on seven algorithmic reasoning tasks, we demonstrate the effectiveness of Think-and-Execute. Our approach better improves LMs' reasoning compared to several strong baselines performing instance-specific reasoning (e.g., CoT and PoT), suggesting the helpfulness of discovering task-level logic. Also, we show that compared to natural language, pseudocode can better guide the reasoning of LMs, even though they are trained to follow natural language instructions.

==> 4_framework.tex <==
\section{Framework (for Prompt Generation)}
While code prompt is efficient in describing reasoning logic, not all people that might use LLMs are proficient in programming languages, which can be a huge huddle for using our method. To this end, we propose our framework that automatically generates code prompt $\mathcal{P}_{machine}$ without human labor. Our framework consists of two LMs, an Instructor  \instructor and a Reasoner \reasoner. In this section, we describe how the Instructor \instructor constructs \machinecodeprompt.

\subsection{Generating an Initial Code Prompt with Meta Prompt}
To generate \machinecodeprompt with \instructor, we prompt the LM with a meta prompt which  consists of 
examplars from other tasks that consist of 
\subsection{Debugging Reasoning Path with Unit Test Results}


==> figure_latex/figure4.tex <==


\begin{figure}
    \centering
    \includegraphics[width=0.99\linewidth]{figure/example_explanation_and_code_prompt.pdf}
    \caption{An example of (a) a generated analysis and (b) a generated \codeprompt for Naviation task~\citep{suzgun2022challenging}. The analysis highlights some key reasoning logic that must be incorporated to solve the task, such as initializing the variables (\eg coordinates and orientation) and keep tracking of them. And the \codeprompt based on the analysis implements the key logic in a pseudocode format and use \texttt{print()} function to explicitly generate the variables. Note that the pseudocode prompt adopts the syntax of Python, but it is not fully executable with a real Python interpreter due to ``Not implemented error: process\_instruction''.}
    \label{fig:analysis_prompt}
\end{figure}

==> prompts/task_classification.tex <==
\begin{figure}
    \begin{small}
        \captionsetup{justification=centering, labelfont=bf, font=small}
        \begin{minted}[fontsize=\footnotesize, frame=lines, framesep=2mm, baselinestretch=1.2, breaklines, breaksymbolleft={}, breaksymbolright={},bgcolor=Box2Color]{text}
Choose between the variables tracking and the free format reasoning which strategy would be more effective than the other one when tackling the last task considering the example task instances and explain why. The variables tracking is effective when the task has multiple instructions or statements to process and need to check the important variables for each of the step. For the free format reasoning, it works well when the task needs a complex or diverse logic that is difficult to be expressed in a specific method. In a free format reasoning step, you don't have to specify the logic, but you should specify an abstract fucntion like 'derive_answer_with_explantion' which outputs both reasons and proper answer for the situation. For the variables tracking step, you should use 'for loop' to process the multiple statements or instructions step by step, 'print()' to output intermediate steps to keep track of changes of variables.

[Example 1]
{example_instances_of_task1}

Reason for the decision & Answer:
{reason_and_answer_for_task1}

...

[Example 4]
{example_instances_of_target_task}

Reason for the decision & Answer:
        \end{minted}
    \end{small}
    \caption{Prompt for classifying the target task}
    \label{fig:prompt:task_classifications}
\end{figure}

==> table/plan_and_solve.tex <==
\begin{table}[t]
\centering
\begin{tabular}{lc}
\toprule
\textbf{Method} & Avg \\
\midrule
Plan-and-Solve & 50.3 \\
\ours & \textbf{53.0}\\

\bottomrule
\end{tabular}
\caption{Comparison with Plan-and-Solve~\citep{wang-etal-2023-plan}.}\label{tab:plan_and_solve}
\end{table}


